Accelerated Proximal Alternating Gradient-Descent-Ascent for Nonconvex Minimax Machine Learning

Alternating gradient-descent-ascent (AltGDA) is an optimization algorithm that has been widely used for model training in various machine learning applications, which aims to solve a nonconvex minimax optimization problem. However, the existing studies show that it suffers from a high computation complexity in nonconvex minimax optimization. In this paper, we develop a single-loop and fast AltGDA-type algorithm that leverages proximal gradient updates and momentum acceleration to solve regularized nonconvex minimax optimization problems. By leveraging the momentum acceleration technique, we prove that the algorithm converges to a critical point in nonconvex minimax optimization and achieves a computation complexity in the order of $\mathcal{O}(\kappa^{\frac{11}{6}}\epsilon^{-2})$, where $\epsilon$ is the desired level of accuracy and $\kappa$ is the problem's condition number. {Such a computation complexity improves the state-of-the-art complexities of single-loop GDA and AltGDA algorithms (see the summary of comparison in \Cref{table1})}. We demonstrate the effectiveness of our algorithm via an experiment on adversarial deep learning.

==> assumption1.tex <==
\section{Proof of the relationship among the statements in Assumption 1}\label{sec_assum1}

We will prove that in \Cref{assum: f}, the item 2 and the statement that $g$ is lower semi-continuous can be derived from the rest of \Cref{assum: f}. 
\begin{proof}
	\noindent Since the sub-level set $\{x: (\Phi+g)(x)\le\alpha\}$ is closed, $\Phi+g$ is lower semi-continuous. Without item 2 and any assumption on $g$, Lemma \Cref{prop_Phiystar} holds which implies continuity of $\Phi$, so $g$ is lower semi-continuous.  
	
	%\noindent If the sub-level set $A=\{x: (\Phi+g)(x)\le0 \}$ is empty, then 0 is a lower bound of $\Phi+g$. Hence, we focus on the case where $A$ is non-empty convex set.\\
	
	\noindent Suppose $\Phi+g$ is not bounded below, then there is a sequence $\{x_t\}_t$ such that $(\Phi+g)(x_t)\le -t$. Since $x_t\in A$ and $A$ is compact, $\{x_n\}$ has at one convergent subsequence $x_{n(t)}\overset{t}{\to} x^*$. Since $\Phi+g$ is lower semi-continuous, $\Phi(x^*)+g(x^*)\le \mathop{\lim\inf}_{n\to\infty} \Phi(x_{n(t)})+g(x_{n(t)})=-\infty$. However, since $\Phi$ is continuous and $g$ is proper, $\Phi(x^*), g(x^*)>-\infty$, is a contradiction. Hence, $\Phi+g$ is not bounded below, that is, the item 2 of \Cref{assum: f} holds
\end{proof}

==> introduction_old_.tex <==
\section{Introduction}
A majority of machine learning applications are naturally formulated as nonconvex optimization due to the complex mechanism of the underlying model. Typical examples include training neural networks in deep learning \cite{Goodfellow2016}, low-rank matrix factorization \cite{RongGe2016,Bhojanapalli2016}, phase retrieval \cite{Candes2015,Zhang2017}, etc. In particular, these machine learning problems take the generic form
\begin{align*}
\min_{\xb\in \RR^d}~~f(\xb), \tag{P}
\end{align*}
where the objective function $f: \RR^d \to \RR$ is a differentiable and nonconvex function, and usually corresponds to the total loss over a set of data samples. 
Traditional first-order algorithms such as gradient descent can produce a solution $\bar{\xb}$ that satisfies the first-order stationary condition, i.e., $\nabla f (\bar{\xb}) = \zero$. However, such first-order stationary condition does not exclude the possibility of approaching a saddle point, which can be a highly suboptimal solution and therefore deteriorate the performance. 

Recently in the machine learning community, there has been an emerging interest in designing algorithms to scape saddle points in nonconvex optimization, and one popular algorithm is the cubic-regularized Newton's algorithm \cite{Nesterov2006,Agarwal2017,Yue2018}, which is also referred to as cubic regularization (CR) for simplicity. Such a second-order method exploits the Hessian information and produces a solution $\bar{\xb}$ for problem (P) that satisfies the second-order stationary condition, i.e., 
$$(\text{second-order stationary}):\quad \nabla f (\bar{\xb}) = \zero, ~\nabla^2 f(\bar{\xb}) \succeq \zero.$$
The second-order stationary condition ensures CR to escape saddle points wherever the corresponding Hessian matrix has a negative eigenvalue (i.e., strict saddle points \cite{Sun2015}). In particular, many nonconvex machine learning problems have been shown to exclude spurious local minima and have only strict saddle points other than global minima \cite{Baldi1989,Sun2017,RongGe2016,zhou2018}. In such a desirable case, CR is guaranteed to find the global minimum for these nonconvex problems. 
To be specific, given a proper parameter $M>0$, CR generates a variable sequence $\{ \xb_{k}\}_k$ via the following update rule
\begin{align}
	\text{(CR)}~ \xb_{k+1} \in \argmin_{\yb \in \RR^d} ~\inner{\yb - \xb_{k}}{\nabla f (\xb_{k})} + \frac{1}{2} (\yb - \xb_{k})^\ttop \nabla^2 f(\xb_{k})  (\yb - \xb_{k}) + \frac{M}{6} \|\yb - \xb_{k}\|^3. \label{eq: CR}
\end{align}
Intuitively, CR updates the variable by minimizing an approximation of the objective function at the current iterate. This approximation is essentially the third-order Taylor's expansion of the objective function. We note that computationally efficient solver has been proposed for solving the above cubic subproblem \cite{Agarwal2017}, and it was shown that the resulting computation complexity of CR to achieve a second-order stationary point serves as the state-of-the-art among existing algorithms that achieve the second-order stationary condition.
%is lower than that of gradient descent to achieve a first-order stationary point.

Several studies have explored the convergence of CR for nonconvex optimization. Specifically, the pioneering work \cite{Nesterov2006} first proposed the CR algorithm and showed that the variable sequence $\{\xb_{k} \}_k$ generated by CR has second-order stationary limit points and converges sub-linearly. Furthermore, the gradient norm along the iterates was shown to converge quadratically (i.e., super-linearly) given an initialization with positive definite Hessian. Moreover, the function value along the iterates was shown to converge super-linearly under a certain gradient dominance condition of the objective function. Recently, \cite{Yue2018} studied the asymptotic convergence rate of CR under the local error bound condition, and established the quadratic convergence of the distance between the variable and the solution set. 
Clearly, these results demonstrate that special geometrical properties (such as the gradient dominance condition and the local error bound) enable much faster convergence rate of CR towards a second-order stationary point. However, these special conditions may fail to hold for generic complex objectives involved in practical applications. Thus, it is desired to further understand the convergence behaviors of CR for optimizing nonconvex functions over a broader spectrum of geometrical conditions.

The Kurdyka-{\L}ojasiewicz (K{\L}) property (see \Cref{sec: pre} for details) \cite{Bolte2007,Bolte2014} serves as such a candidate. As described in \Cref{sec: pre}, the \KL property captures a broad spectrum of the local geometries that a nonconvex function can have and is parameterized by a parameter $\theta$ that changes over its allowable range.  In fact, the \KL property has been shown to hold ubiquitously for most practical functions (see \Cref{sec: pre} for a list of examples). 
The \KL property has been exploited extensively to analyze the convergence rate of various {\em first-order} algorithms for nonconvex optimization, e.g., gradient method \cite{Attouch2009,Li2017}, alternating minimization \cite{Bolte2014} and distributed gradient methods \cite{Zhou2016}.
But it has not been exploited to establish the {\em convergence rate} of second-order algorithms towards second-order stationary points.  
In this paper, we exploit the \KL property of the objective function to provide a comprehensive study of the convergence rate of CR for nonconvex optimization. We anticipate our study to substantially advance the existing understanding of the convergence of CR to a much broader range of nonconvex functions. We summarize our contributions as follows.
\vspace{-5pt}
\subsection{Our Contributions}
\vspace{-5pt}
We characterize the convergence rate of CR locally towards second-stationary points for nonconvex optimization under the \KL property of the objective function. Our results also compare and contrast the different order-level of guarantees that \KL yields between the first and second-order algorithms.
Also, our analysis characterizes the convergence property for a range of \KL parameter $\theta$,  which requires the development of different recursive inequalities for various cases.

\textbf{Gradient norm \& least eigenvalue of Hessian:}
We characterize the asymptotic convergence rates of the sequence of gradient norm $\{\|\nabla f(\xb_{k})\| \}_k$ and the sequence of the least eigenvalue of Hessian $\{\lambda_{\min} (\nabla^2 f(\xb_{k}))\}_k$ generated by CR. We show that CR meets the second-order stationary condition at a (super)-linear rate in the parameter range $\theta \in [\frac{1}{3}, 1]$ for the \KL property, while the convergence rates become sub-linearly in the parameter range $\theta \in (0, \frac{1}{3})$ for the \KL property.

\textbf{Function value gap \& variable distance:} 
We characterize the asymptotic convergence rates of the function value sequence $\{f(\xb_{k})\}_k$ and the variable sequence $\{\xb_{k}\}_k$ to the function value and the variable of a second-order stationary point, respectively. The obtained convergence rates range from sub-linearly to super-linearly depending on the parameter $\theta$ associated with the \KL property. Our convergence results generalize the existing ones established in \cite{Nesterov2006} corresponding to special cases of $\theta$ to the full range of $\theta$. Furthermore, these types of convergence rates for CR are orderwise faster than the corresponding convergence rates of the first-order gradient descent algorithm in various regimes of the \KL parameter $\theta$ (see \Cref{table: 1} and \Cref{table: 2}  for the comparisons). 

Based on the \KL property, we establish a generalized local error bound condition (referred to as the \KL error bound). The \KL error bound further leads to characterization of the convergence rate of distance between the variable and the solution set, which ranges from sub-linearly to super-linearly depending on the parameter $\theta$ associated with the \KL property.
This result generalizes the existing one established in \cite{Yue2018} corresponding to a special case of $\theta$ to the full range of $\theta$. 


\vspace{-5pt}
\subsection{Related Work}
\vspace{-5pt}
\textbf{Cubic regularization:} CR algorithm was first proposed in \cite{Nesterov2006}, in which the authors analyzed the convergence of CR to second-order stationary points for nonconvex optimization. In \cite{Nesterov2008}, the authors established the sub-linear convergence of CR for solving convex smooth problems, and they further proposed an accelerated version of CR with improved sub-linear convergence. Recently, \cite{Yue2018} studied the asymptotic convergence properties of CR under the error bound condition, and established the quadratic convergence of the iterates. Several other works proposed different methods to solve the cubic subproblem of CR, e.g., \cite{Agarwal2017,Carmon2016,Cartis2011a}.


\textbf{Inexact-cubic regularization:} 
Another line of work aimed at improving the computation efficiency of CR by solving the cubic subproblem with inexact gradient and Hessian information. In particular, \cite{Saeed2017,Jin2017} proposed an inexact CR for solving convex problem and nonconvex problems, respectively. Also, \cite{Cartis2011b} proposed an adaptive inexact CR for nonconvex optimization, whereas \cite{Jiang2017} further studied the accelerated version for convex optimization. Several studies explored subsampling schemes to implement inexact CR algorithms, e.g., \cite{kohler2017,Xu2017,Zhou2018,Wang2018}. 


\textbf{\KL property:} The \KL property was first established in \cite{Bolte2007}, and was then widely applied to characterize the asymptotic convergence behavior for various first-order algorithms for nonconvex optimization \cite{Attouch2009,Li2017,Bolte2014,Zhou2016,Zhou_2017a}. The \KL property was also exploited to study the convergence of second-order algorithms such as generalized Newton's method \cite{Frankel2015} and the trust region method \cite{Noll2013}. However, these studies did not characterize the convergence rate and the studied methods cannot guarantee to converge to second-order stationary points, whereas this paper provides this type of results.

\textbf{First-order algorithms that escape saddle points:} Many first-order algorithms are proved to achieve second-order stationary points for nonconvex optimization. For example, online stochastic gradient descent \cite{Ge2015}, perturbed gradient descent \cite{Jin2017}, gradient descent with negative curvature \cite{Carmon2016,Liu2017} and other stochastic algorithms \cite{Zhu2017}.



==> litnotes.tex <==
\section{Lits: To delete}
\cite{boct2020alternating}: stochastic proximal alternating-GDA, nonconvex-strongly concave, nonconvex-concave.\\

Deterministic iteration complexity  $\mathcal{O}(\kappa^2\epsilon^{-2})$ for nonconvex strongly concave.

Claim the importance of single-loop: ``Despite superior theoretical performance these methods have not been as popular in practice, especially in the training of GANs where single loop methods are still state-of-the-art [\cite{bailey2020finite}, 7\cite{daskalakis2018training}, 13, \cite{gidel2019negative}, 16, 20, 25].''??

The alternating-GDA has more desired convergence properties than those of the simultaneous-GDA [\cite{boct2020alternating,bailey2020finite,gidel2019negative,xu2020unified}]

\cite{yadav2018stabilizing}: Stochastic Alternating GDA+momentum on generator (descent) for GAN. Convergence rate under convex-concavity and bounded expected stochastic gradients. 

\cite{xu2020unified}: Projected single-loop alternating GDA achieves iteration complexity. States that nested-loop algorithms are relatively complicated to be implemented and that single-loop algorithms are more popular in practice due to their simplicity.

Single-loop [23]

\cite{goodfellow2014generative}: GAN uses single-loop alternating GDA. 

\cite{daskalakis2018training}: Training Wasserstein GANs with single-loop Optimistic Mirror Descent. 

\cite{gidel2019negative}: Investigate gradient-based simultaneous VS alternating update with negative momentum (we put to related work) on adversarial games (aiming at Nash equilibrium of multiple objectives). alternating update has better convergence in that only alternating update with negative momentum can converge. Fig. 1 Lists Momentum works in training GANs. ??

\cite{mirza2014conditional,radford2015unsupervised,denton2015deep}: Momentum in GAN. 

\cite{bailey2020finite}: Single-loop alternating GDA applied to Bilinear Zero-Sum Game, ``alternating updates also does not require competing agents to coordinate (in zero-sum game)''

\cite{shafahi2019adversarial}: Single-loop alternating for adversarial training, not exactly GDA but mirror descent. No momentum. 



==> proposition1proof.tex <==
\section{Proof of \Cref{prop_Phiystar}} \label{sec_prop1proof}

\propphy*
\begin{proof}
	We first prove item 1.
	Since $f(x,y)$ is strongly concave in $y$ for every $x$ and $h(y)$ is convex, the mapping $y^*(x)=\arg\max _{y\in \mathbb{R}^{n}}f(x,y)-h(y)$ is uniquely defined. We first show that $y^*(x)$ is a Lipschitz mapping. Consider two arbitrary points $x_1, x_2$. The optimality conditions of $y^*(x_1)$ and $y^*(x_2)$ imply that
	\begin{align}
	\inner{y - y^*(x_1)}{{\nabla_2 f}(x_1, y^*(x_1)) - u_1} &\le 0, \quad \forall y\in \mathbb{R}^{n}, u_1\in \partial h(y^*(x_1)), \label{eq: 6}\\
	\inner{y - y^*(x_2)}{{\nabla_2 f}(x_2, y^*(x_2)) - u_2} &\le 0, \quad \forall y\in \mathbb{R}^{n}, u_2\in \partial h(y^*(x_2)).\label{eq: 7}
	\end{align}
	Setting $y = y^*(x_2)$ in \cref{eq: 6}, $y = y^*(x_1)$ in \cref{eq: 7} and summing up the two inequalities, 	we obtain that
	\begin{align}
	\inner{y^*(x_2)- y^*(x_1)}{{\nabla_2 f}(x_1, y^*(x_1)) - {\nabla_2 f}(x_2, y^*(x_2)) - u_1 + u_2} &\le 0.
	\end{align}
	Since $\partial h$ is a monotone operator (by convexity), we know that $\inner{u_2 - u_1}{y^*(x_2)- y^*(x_1)} \ge 0$. Hence, the above inequality further implies that  
	\begin{align}
	\inner{y^*(x_2)- y^*(x_1)}{{\nabla_2 f}(x_1, y^*(x_1)) - {\nabla_2 f}(x_2, y^*(x_2))} &\le 0.
	\end{align}
	Next, by strong concavity of $f(x_1, \cdot)$, we have that
	\begin{align}
	\inner{y^*(x_2)- y^*(x_1)}{{\nabla_2 f}(x_1, y^*(x_2)) - {\nabla_2 f}(x_1, y^*(x_1))} + \mu \|y^*(x_1) - y^*(x_2)\|^2&\le 0.
	\end{align}
	Adding up the above two inequalities yields that
	\begin{align}
	\mu \|y^*(x_1) - y^*(x_2)\|^2&\le \inner{y^*(x_2)- y^*(x_1)}{{\nabla_2 f}(x_2, y^*(x_2)) - {\nabla_2 f}(x_1, y^*(x_2))} \nonumber\\
	&\le \|y^*(x_2)- y^*(x_1)\| \|{\nabla_2 f}(x_2, y^*(x_2)) - {\nabla_2 f}(x_1, y^*(x_2))\| \nonumber\\
	&\le L\|y^*(x_2)- y^*(x_1)\| \|x_2 - x_1\|. \nonumber
	\end{align}
	The above inequality shows that $\|y^*(x_1) - y^*(x_2)\| \le \kappa \|x_2 - x_1\|$, and item 1 is proved. 
	
	Next, we will prove item 2.
%	Next, we prove $\nabla\Phi(x)=\nabla_1 f[x,y^*(x)]$ in item 2 by verifying the condition of the Danskin theorem \cite{bernhard1995theorem}, that is, we aim to find a compact set $B\subset\mathbb{R}^{n}$ such that $y^*(x)=\arg\max_{y\in B}f(x,y)-h(y)$ and the functions  $f(x,y)-h(y)$ and $\nabla_1 f(x,y)$ are continuous in $(x,y)\in \mathbb{R}^m \times B$. \\
	
%	Since $h$ is convex and proper, $h$ is continuous on the nonempty convex set $A:=\{y\in\mathbb{R}^{n}: h(y)\in\mathbb{R}\}$ (see Corollary 10.1.1 of \cite{rockafellar1970convex}), and thus $f(x,y)-h(y)$ is continuous in  $(x,y)\in \mathbb{R}^m \times A$. $\nabla_1 f(x,y)$ is $L$-lipschitz continuous by \Cref{assum: f}. Since $A\subset \mathbb{R}^{n}$ and $\mathbb{R}^{n}$ is compact, $A$ is a bounded but possibly non-compact set. \\
	
	Consider $A_n=\{y^*(x): x\in\mathbb{R}^m, \|x\|\le n\}\subset \mathbb{R}^{n}$. Since $\Phi+g$ is lower bounded by \Cref{assum: f}, we have for any $x\in\mathbb{R}^m$, $\Phi(x)=f(x,y^*(x))-h(y^*(x))>-\infty$ and hence $h(y^*(x))<+\infty$. Hence, based on Corollary 10.1.1 of \cite{rockafellar1970convex}, $h(y)$ is continuous on $A_n$ and thus $f(x,y)-h(y)$ is continuous in $(x,y)\in \mathbb{R}^m \times A_n$. Also, $\nabla_1 f(x,y)$ is continuous in $(x,y)\in \mathbb{R}^m \times A_n$ since $f$ is $L$-smooth. For any sequence $\{x_k\}$ such that $\|x_k\| \le n$ and $y^*(x_k) \to y\in\mathbb{R}^{n}$, $y=y^*(x')$ for any limit point $x'$ of $\{x_k\}$ (there is at least one such limit point since $\|x_k\| \le n$) since we have proved that $y^*$ is continuous. As $\|x'\|\le n$, $y\in A_n$. Hence, $A_n$ is closed. As $A_n$ is included in bounded $\mathbb{R}^{n}$, $A_n$ is compact. Therefore, based on the Danskin theorem \cite{bernhard1995theorem}, the function $\Phi_n(x):=\arg\max_{y\in A_n}f(x,y)-h(y)$ is differntialable with $\nabla \Phi_n(x)=\nabla_1 f(x,y^*(x))$. On one hand, $\Phi_n(x) \le \Phi(x)$ since $A_n\subset \mathbb{R}^{n}$. On the other hand, when $\|x\|\le n$, $y^*(x)\in A_n$, so $\Phi(x)=f(x,y^*(x))-h(y^*(x)) \le \Phi_n(x)$. Hence, when $\|x\|\le n$, $\Phi(x)=\Phi_n(x)$ and thus $\nabla \Phi(x)=\nabla \Phi_n(x)=\nabla_1 f(x,y^*(x))$. Since $n$ can be arbitrarily large, $\nabla \Phi(x)=\nabla_1 f(x,y^*(x))$ for any $x\in\mathbb{R}^m$. 
	
	Next, consider any $x_1, x_2\in\mathbb{R}^m$, we obtain that
	\begin{align}
		\|\nabla\Phi(x_2)-\nabla\Phi(x_1)\|=& \|\nabla_1 f(x_2,y^*(x_2))-\nabla_1 f(x_1,y^*(x_1))\|\nonumber\\
		\le& L\|x_2-x_1\|+L\|y^*(x_2)-y^*(x_1)\|\nonumber\\
		\le& L\|x_2-x_1\|+L\kappa\|x_2-x_1\|\nonumber\\
		=&L(1+\kappa)\|x_2-x_1\|,\nonumber
	\end{align}
	which implies that $\Phi(x)$ is $L(1+\kappa)$-smooth. 
	
%	{For any $x_1\in\mathbb{R}^m$, $0\in \nabla_2 f[x_1,y^*(x_1)]-\partial h[y^*(x_1)]\Rightarrow \nabla_2 f[x_1,y^*(x_1)]\in\partial h[y^*(x_1)]$. Hence, for any $x_1, x_2\in\mathbb{R}^m$,}
%	\begin{align}
%	h[y^*(x_2)]-h[y^*(x_1)]\ge \nabla_2 f[x_1,y^*(x_1)]^{\top}[y^*(x_2)-y^*(x_1)]\label{hconvex}
%	\end{align}
%	
%	Then, we obtain that
%	\begin{align}
%	&\Phi(x_2)-\Phi(x_1)\nonumber\\
%	&=f[x_2,y^*(x_2)]-f[x_1,y^*(x_1)]-h[y^*(x_2)]+h[y^*(x_1)]\nonumber\\
%	&\stackrel{(i)}{\le}f[x_2,y^*(x_2)]-f[x_1,y^*(x_1)]-\nabla_2 f[x_1,y^*(x_1)]^{\top}[y^*(x_2)-y^*(x_1)]\nonumber\\
%	&\stackrel{(ii)}{=}\nabla_1 f[x_1,y^*(x_1)]^{\top}(x_2-x_1)+o[\|x_2-x_1\|+\|y^*(x_2)-y^*(x_1)\|]\nonumber\\
%	&\stackrel{(iii)}{=}\nabla_1 f[x_1,y^*(x_1)]^{\top}(x_2-x_1)+o(\|x_2-x_1\|)\label{diff_Phi}
%	\end{align}
%	where (i) uses eq. \eqref{hconvex}, (ii) uses Taylor expansion of $f$ at the point $[x_1,y^*(x_1)]$, (iii) uses the Lipschitz property of $y^*(x)$. 
%	
%	Since $\nabla_1 f$ and $y^*$ are Lipschitz continuous with parameters $L$ and $\kappa$ respectively, we have
%	\begin{align}
%	\|\nabla_1 f[x_1,y^*(x_1)]-\nabla_1 f[x_2,y^*(x_2)]\|\le& L[\|x_2-x_1\|+\|y^*(x_2)-y^*(x_1)\|]\nonumber\\
%	\le& L(1+\kappa)\|x_2-x_1\| \label{f1_smooth}
%	\end{align} 
%	
%	Hence,
%	\begin{align}
%	&\Big[\nabla_1 f[x_1,y^*(x_1)]-\nabla_1 f[x_2,y^*(x_2)]\Big]^{\top}(x_2-x_1)\nonumber\\
%	&\le \|\nabla_1 f[x_1,y^*(x_1)]-\nabla_1 f[x_2,y^*(x_2)]\|\|x_2-x_1\|\nonumber
%	\\
%	&\le L(1+\kappa)\|x_2-x_1\|^2, \nonumber
%	\end{align}
%	which implies that
%	\begin{align}
%	\nabla_1 f[x_1,y^*(x_1)]^{\top}(x_2-x_1)=\nabla_1 f[x_2,y^*(x_2)]^{\top}(x_2-x_1)+o(\|x_2-x_1\|)\label{f1_replace}
%	\end{align} 
%	Substituting eq. \eqref{f1_replace} into eq. \eqref{diff_Phi} yields that
%	\begin{align}
%	\Phi(x_2)-\Phi(x_1)\le \nabla_1 f[x_2,y^*(x_2)]^{\top}(x_2-x_1)+o(\|x_2-x_1\|) \label{diff_Phi2}
%	\end{align}
%	By switching $x_1$ and $x_2$ in eq. \eqref{diff_Phi2}, we obtain
%	\begin{align}
%	\Phi(x_1)-\Phi(x_2)\le -\nabla_1 f[x_1,y^*(x_1)]^{\top}(x_2-x_1)+o(\|x_2-x_1\|) \label{diff_Phi3}
%	\end{align}
%	Then, eqs. \eqref{diff_Phi} \& \eqref{diff_Phi3} imply that
%	\begin{align}
%	\Phi(x_2)-\Phi(x_1)=\nabla_1 f[x_1,y^*(x_1)]^{\top}(x_2-x_1)+o(\|x_2-x_1\|),
%	\end{align}
%	{which further implies that $\Phi(x)$ is differentiable with $\nabla\Phi(x)=\nabla_1 f[x_1,y^*(x_1)]$. Hence, eq. \eqref{f1_smooth} implies that $\Phi(x)$ is $L(1+\kappa)$-smooth, which proves the item 2.}


\end{proof}
